Robust Regression with Compositional Covariates

Many biological high-throughput data sets, such as targeted amplicon-based and metagenomic sequencing data, are compositional in nature. A common exploratory data analysis task is to infer statistical associations between the high-dimensional microbial compositions and habitat- or host-related covariates. We propose a general robust statistical regression framework, RobRegCC (Robust Regression with Compositional Covariates), which extends the linear log-contrast model by a mean shift formulation for capturing outliers. RobRegCC includes sparsity-promoting convex and non-convex penalties for parsimonious model estimation, a data-driven robust initialization procedure, and a novel robust cross-validation model selection scheme. We show RobRegCC's ability to perform simultaneous sparse log-contrast regression and outlier detection over a wide range of simulation settings and provide theoretical non-asymptotic guarantees for the underlying estimators. To demonstrate the seamless applicability of the workflow on real data, we consider a gut microbiome data set from HIV patients and infer robust associations between a sparse set of microbial species and host immune response from soluble CD14 measurements. All experiments are fully reproducible and available on GitHub at https://github.com/amishra-stats/robregcc.

==> table.tex <==
\begin{table}[H]

\caption{\label{tab:sequal6}Demo table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabu} to \linewidth {>{\raggedleft}X>{\raggedleft}X>{\raggedleft}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
\multicolumn{3}{c}{\textbf{ }} & \multicolumn{3}{c}{\textbf{[A]}} & \multicolumn{3}{c}{\textbf{[H]}} & \multicolumn{3}{c}{\textbf{[S]}} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9} \cmidrule(l{3pt}r{3pt}){10-12}
L & p & O & FN & FP & HM & FN & FP & HM & FN & FP & HM\\
\midrule
\rowcolor{gray!6}   &  & 10 & 0.01 (0.10) & 27.89 (10.86) & 27.90 (10.83) & 0.01 (0.10) & 14.16 (8.40) & 14.17 (8.40) & 0.00 (0.00) & 31.89 (13.36) & 31.89 (13.36)\\

 &  & 20 & 0.00 (0.00) & 20.96 (9.70) & 20.96 (9.70) & 0.06 (0.28) & 11.49 (6.58) & 11.55 (6.52) & 0.00 (0.00) & 30.84 (10.75) & 30.84 (10.75)\\

\rowcolor{gray!6}   & \multirow{-3}{*}{\raggedleft\arraybackslash 100} & 40 & 0.04 (0.20) & 10.50 (6.52) & 10.54 (6.51) & 0.44 (1.24) & 6.21 (4.75) & 6.65 (4.51) & 0.00 (0.00) & 24.72 (7.72) & 24.72 (7.72)\\

 &  & 10 & 0.00 (0.00) & 29.30 (10.43) & 29.30 (10.43) & 0.00 (0.00) & 25.14 (9.85) & 25.14 (9.85) & 0.00 (0.00) & 21.43 (9.29) & 21.43 (9.29)\\

\rowcolor{gray!6}   &  & 20 & 0.01 (0.10) & 21.69 (10.22) & 21.70 (10.20) & 0.00 (0.00) & 26.85 (10.20) & 26.85 (10.20) & 0.00 (0.00) & 18.90 (7.72) & 18.90 (7.72)\\

\multirow{-6}{*}{\raggedleft\arraybackslash 0} & \multirow{-3}{*}{\raggedleft\arraybackslash 300} & 40 & 0.03 (0.17) & 9.80 (5.94) & 9.83 (5.92) & 0.19 (0.66) & 23.89 (6.83) & 24.08 (6.60) & 0.18 (0.54) & 15.07 (5.41) & 15.25 (5.28)\\

\rowcolor{gray!6}   &  & 10 & 0.00 (0.00) & 28.89 (10.63) & 28.89 (10.63) & 0.06 (0.60) & 15.68 (8.78) & 15.74 (8.69) & 0.45 (0.88) & 31.39 (12.22) & 31.84 (11.95)\\

 &  & 20 & 0.03 (0.30) & 20.19 (8.61) & 20.22 (8.60) & 0.31 (1.47) & 12.03 (7.58) & 12.34 (7.33) & 2.76 (2.91) & 27.40 (12.32) & 30.16 (11.63)\\

\rowcolor{gray!6}   & \multirow{-3}{*}{\raggedleft\arraybackslash 100} & 40 & 0.87 (3.36) & 8.26 (5.75) & 9.13 (6.04) & 4.41 (8.67) & 7.32 (5.65) & 11.73 (8.04) & 8.93 (6.20) & 22.37 (9.13) & 31.30 (9.29)\\

 &  & 10 & 0.01 (0.10) & 29.40 (12.26) & 29.41 (12.24) & 0.01 (0.10) & 28.73 (11.38) & 28.74 (11.39) & 0.76 (0.98) & 23.52 (11.45) & 24.27 (11.25)\\

\rowcolor{gray!6}   &  & 20 & 0.01 (0.10) & 22.17 (9.85) & 22.18 (9.85) & 0.20 (1.24) & 30.68 (11.31) & 30.88 (11.01) & 5.02 (2.92) & 18.25 (9.24) & 23.27 (8.59)\\

\multirow{-6}{*}{\raggedleft\arraybackslash 1} & \multirow{-3}{*}{\raggedleft\arraybackslash 300} & 40 & 0.79 (2.54) & 9.72 (5.88) & 10.51 (5.55) & 5.83 (6.77) & 18.14 (8.59) & 23.98 (5.75) & 15.62 (2.77) & 17.30 (7.38) & 32.92 (5.77)\\
\bottomrule
\end{tabu}}
\end{table}

==> table6.tex <==
\begin{table}[H]

\caption{\label{tab:sequal6}Comparison of RobRegCC model with the hard-ridge [H], the Elastic Net [S], and the adaptive Elastic Net [A] penalty function in simulation setting with moderate outliers (n =200, s = 6) using outlier identification measures  false negative (FN), false positive (FP) and hamming distance (HM).\\}
\centering
\resizebox{\linewidth}{!}{
\fontsize{8}{10}\selectfont
\begin{tabu} to \linewidth {>{\raggedleft}X>{\raggedleft}X>{\raggedleft}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
\multicolumn{3}{c}{\textbf{ }} & \multicolumn{3}{c}{\textbf{[A]}} & \multicolumn{3}{c}{\textbf{[H]}} & \multicolumn{3}{c}{\textbf{[S]}} & \multicolumn{3}{c}{\textbf{[NR]}} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9} \cmidrule(l{3pt}r{3pt}){10-12} \cmidrule(l{3pt}r{3pt}){13-15}
\rowcolor{gray!6}  L & p & O & FN & FP & Er($\bbeta$) & FN & FP & Er($\bbeta$) & FN & FP & Er($\bbeta$) & FN & FP & Er($\bbeta$)\\
\midrule
0 & 100 & 10 & 0.00 & 2.24 & 0.10 & 0.00 & 1.27 & 0.07 & 0.00 & 4.47 & 0.14 & -- & -- & 0.40\\
\rowcolor{gray!6}  0 & 100 & 20 & 0.00 & 1.70 & 0.09 & 0.00 & 0.42 & 0.05 & 0.00 & 4.55 & 0.13 & -- & -- & 0.52\\
0 & 100 & 40 & 0.00 & 1.10 & 0.09 & 1.20 & 0.00 & 0.15 & 0.00 & 3.88 & 0.14 & -- & -- & 0.61\\
\hline
\rowcolor{gray!6}  0 & 300 & 10 & 0.00 & 4.28 & 0.37 & 0.00 & 2.93 & 0.28 & 0.00 & 7.39 & 0.45 & -- & -- & 0.19\\
0 & 300 & 20 & 0.00 & 3.96 & 0.33 & 0.00 & 2.54 & 0.29 & 0.00 & 5.27 & 0.40 & -- & -- & 0.25\\
\addlinespace
\rowcolor{gray!6}  0 & 300 & 40 & 0.00 & 2.25 & 0.29 & 1.44 & 0.37 & 0.46 & 0.00 & 3.82 & 0.36 & -- & -- & 0.30\\
\hline
1 & 100 & 10 & 0.00 & 2.39 & 0.12 & 0.00 & 1.20 & 0.08 & 0.23 & 4.46 & 0.22 & -- & -- & 0.61\\
\rowcolor{gray!6}  1 & 100 & 20 & 0.00 & 2.05 & 0.11 & 0.29 & 0.67 & 0.10 & 4.35 & 3.91 & 0.55 & -- & -- & 0.85\\
1 & 100 & 40 & 4.75 & 0.47 & 0.42 & 4.04 & 0.00 & 0.41 & 14.37 & 2.48 & 0.97 & -- & -- & 1.11\\
\hline
\rowcolor{gray!6}  1 & 300 & 10 & 0.00 & 4.32 & 0.36 & 0.00 & 1.90 & 0.26 & 1.26 & 5.06 & 0.80 & -- & -- & 0.24\\
\addlinespace
1 & 300 & 20 & 0.00 & 3.16 & 0.45 & 0.00 & 1.30 & 0.24 & 6.80 & 4.08 & 1.82 & -- & -- & 0.33\\
\rowcolor{gray!6}  1 & 300 & 40 & 13.71 & 1.35 & 2.16 & 1.86 & 0.31 & 0.74 & 19.14 & 3.91 & 2.78 & -- & -- & 0.43\\
\bottomrule
\end{tabu}}
\end{table}

==> table8.tex <==
\begin{table}[H]

\caption{\label{tab:sequal8}Comparison of RobRegCC model with the hard-ridge [H], the Elastic Net [S], and the adaptive Elastic Net [A] penalty function in simulation setting with high outliers (n =200, s = 8) using outlier identification measures  false negative (FN), false positive (FP) and hamming distance (HM).\\}
\centering
\resizebox{\linewidth}{!}{
\fontsize{8}{10}\selectfont
\begin{tabu} to \linewidth {>{\raggedleft}X>{\raggedleft}X>{\raggedleft}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
\multicolumn{3}{c}{\textbf{ }} & \multicolumn{3}{c}{\textbf{[A]}} & \multicolumn{3}{c}{\textbf{[H]}} & \multicolumn{3}{c}{\textbf{[S]}} & \multicolumn{3}{c}{\textbf{[NR]}} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9} \cmidrule(l{3pt}r{3pt}){10-12} \cmidrule(l{3pt}r{3pt}){13-15}
\rowcolor{gray!6}  L & p & O & FN & FP & Er($\bbeta$) & FN & FP & Er($\bbeta$) & FN & FP & Er($\bbeta$) & FN & FP & Er($\bbeta$)\\
\midrule
0 & 100 & 0 & 1.00 & 3.63 & 0.12 & 1.00 & 2.46 & 0.08 & 1.00 & 5.46 & 0.14 & -- & -- & 0.00\\
\rowcolor{gray!6}  0 & 100 & 10 & 0.00 & 2.96 & 0.11 & 0.00 & 1.10 & 0.06 & 0.00 & 4.88 & 0.13 & -- & -- & 0.55\\
0 & 100 & 20 & 0.00 & 1.66 & 0.08 & 0.00 & 0.90 & 0.05 & 0.00 & 4.57 & 0.14 & -- & -- & 0.68\\
\rowcolor{gray!6}  0 & 100 & 40 & 0.00 & 0.95 & 0.06 & 0.00 & 0.00 & 0.04 & 0.00 & 3.56 & 0.14 & -- & -- & 0.73\\
\hline
0 & 300 & 0 & 1.00 & 7.38 & 0.49 & 1.00 & 6.50 & 0.43 & 1.00 & 7.93 & 0.47 & -- & -- & 0.00\\
\addlinespace
\rowcolor{gray!6}  0 & 300 & 10 & 0.00 & 4.55 & 0.35 & 0.00 & 2.86 & 0.29 & 0.00 & 5.73 & 0.38 & -- & -- & 0.22\\
0 & 300 & 20 & 0.00 & 4.08 & 0.36 & 0.00 & 1.68 & 0.26 & 0.00 & 6.28 & 0.47 & -- & -- & 0.29\\
\rowcolor{gray!6}  0 & 300 & 40 & 0.00 & 1.49 & 0.19 & 0.00 & 0.49 & 0.12 & 0.00 & 2.85 & 0.33 & -- & -- & 0.35\\
\hline
1 & 100 & 10 & 0.00 & 2.46 & 0.10 & 0.00 & 1.68 & 0.08 & 0.00 & 4.47 & 0.15 & -- & -- & 0.80\\
\rowcolor{gray!6}  1 & 100 & 20 & 0.00 & 1.71 & 0.09 & 0.00 & 1.02 & 0.06 & 2.96 & 2.94 & 0.52 & -- & -- & 1.07\\
\addlinespace
1 & 100 & 40 & 0.00 & 0.64 & 0.08 & 0.18 & 0.35 & 0.18 & 13.39 & 2.67 & 1.36 & -- & -- & 1.42\\
\hline
\rowcolor{gray!6}  1 & 300 & 10 & 0.00 & 3.78 & 0.33 & 0.00 & 2.34 & 0.24 & 0.19 & 4.55 & 0.71 & -- & -- & 0.32\\
1 & 300 & 20 & 0.00 & 2.29 & 0.25 & 0.00 & 0.91 & 0.15 & 5.65 & 3.44 & 2.00 & -- & -- & 0.42\\
\rowcolor{gray!6}  1 & 300 & 40 & 2.46 & 0.57 & 1.16 & 0.00 & 0.00 & 0.08 & 18.60 & 2.97 & 3.21 & -- & -- & 0.54\\
\bottomrule
\end{tabu}}
\end{table}

==> table_appl1.tex <==
\begin{table}[H]

\caption{\label{tab:appl6}Comparison of RobRegCC model with the hard-ridge [H], the Elastic Net [S], and the adaptive Elastic Net [A] penalty function in soil PH data application  with moderate outliers (s = 3) using outlier identification measures  false negative (FN), false positive (FP) and hamming distance (HM).\\}
\centering
\resizebox{\linewidth}{!}{
\fontsize{7.5}{9.5}\selectfont
\begin{tabu} to \linewidth {>{\raggedleft}X>{\raggedleft}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\bfseries}l}
\toprule
\multicolumn{2}{c}{\textbf{ }} & \multicolumn{4}{c}{\textbf{[A]}} & \multicolumn{4}{c}{\textbf{[H]}} & \multicolumn{4}{c}{\textbf{[S]}} & \multicolumn{1}{c}{\textbf{[NR]}} \\
\cmidrule(l{3pt}r{3pt}){3-6} \cmidrule(l{3pt}r{3pt}){7-10} \cmidrule(l{3pt}r{3pt}){11-14} \cmidrule(l{3pt}r{3pt}){15-15}
\rowcolor{gray!6}  L & O & FN & $\M{FP}_1$ & $\M{FP}_2$ & Er($\bbeta$) & FN & $\M{FP}_1$ & $\M{FP}_2$ & Er($\bbeta$) & FN & $\M{FP}_1$ & $\M{FP}_2$ & Er($\bbeta$) & Er($\bbeta$)\\
\midrule
0 & 4 & 1.10 & 0.00 & 0.00 & 0.73 & 1.87 & 0.46 & 0.00 & 0.80 & 0.47 & 1.13 & 0.00 & 0.56 & 1.32\\
\rowcolor{gray!6}  0 & 9 & 1.36 & 0.91 & 0.00 & 0.99 & 3.81 & 1.08 & 0.00 & 1.52 & 1.10 & 0.75 & 0.00 & 0.82 & 1.41\\
1 & 4 & 1.26 & 0.26 & 0.00 & 1.21 & 1.92 & 0.09 & 0.00 & 1.21 & 1.05 & 0.05 & 0.00 & 0.98 & 1.40\\
\rowcolor{gray!6}  1 & 9 & 2.52 & 0.25 & 0.00 & 1.69 & 3.49 & 1.54 & 0.00 & 1.90 & 1.95 & 1.47 & 0.00 & 1.82 & 1.58\\
\bottomrule
\end{tabu}}
\end{table}

==> table_applF.tex <==
\begin{table}[H]

\caption{\label{tab:applF}Comparison of the non-robust [NR] model and the robust model, i.e.,  RobRegCC with the hard-ridge [H], the Elastic Net [E], and the adaptive Elastic Net [A] penalty function, in the microbiome association study using soil pH data with actively induced O outliers. Models are evaluated using outlier identification measures false negative (FN) and false positive (FP), and the estimation error measure Er($\bbeta$). Here $\M{FP}_1$ and $\M{FP}_2$ refers to the pre and post false positive  measures. \\}
\centering
\resizebox{\linewidth}{!}{
\fontsize{7.5}{9.5}\selectfont
\begin{tabu} to \linewidth {>{\raggedleft}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\bfseries}l>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\bfseries}l>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\bfseries}l>{\bfseries}l}
\toprule
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{4}{c}{\textbf{[A]}} & \multicolumn{4}{c}{\textbf{[H]}} & \multicolumn{4}{c}{\textbf{[E]}} & \multicolumn{1}{c}{\textbf{[NR]}} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9} \cmidrule(l{3pt}r{3pt}){10-13} \cmidrule(l{3pt}r{3pt}){14-14}
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{$\bgamma$} & \multicolumn{1}{c}{$\bbeta$} & \multicolumn{3}{c}{$\bgamma$} & \multicolumn{1}{c}{$\bbeta$} & \multicolumn{3}{c}{$\bgamma$} & \multicolumn{1}{c}{$\bbeta$} & \multicolumn{1}{c}{$\bbeta$} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-8} \cmidrule(l{3pt}r{3pt}){9-9} \cmidrule(l{3pt}r{3pt}){10-12} \cmidrule(l{3pt}r{3pt}){13-13} \cmidrule(l{3pt}r{3pt}){14-14}
\rowcolor{gray!6}  O & FN & $\M{FP}_1$ & $\M{FP}_2$ & Er & FN & $\M{FP}_1$ & $\M{FP}_2$ & Er & FN & $\M{FP}_1$ & $\M{FP}_2$ & Er & Er\\
\midrule
0 & 0.00 & 2.06 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 4.00 & 0.00 & 0.00 & 0.00\\
\rowcolor{gray!6}  4 & 0.00 & 0.00 & 0.00 & 0.07 & 1.14 & 0.00 & 0.00 & 0.08 & 0.00 & 0.00 & 0.00 & 0.07 & 0.21\\
9 & 0.00 & 0.00 & 0.00 & 0.09 & 2.36 & 0.00 & 0.00 & 0.16 & 0.00 & 0.91 & 0.00 & 0.08 & 0.33\\
\bottomrule
\end{tabu}}
\end{table}
